Data curation via joint example selection further accelerates multimodal learning

Data curation is an essential component of large-scale pretraining. In this work, we demonstrate that jointly selecting batches of data is more effective for learning than selecting examples independently. Multimodal contrastive objectives expose the dependencies between data and thus naturally yield criteria for measuring the joint learnability of a batch. We derive a simple and tractable algorithm for selecting such batches, which significantly accelerate training beyond individually-prioritized data points. As performance improves by selecting from larger super-batches, we also leverage recent advances in model approximation to reduce the associated computational overhead. As a result, our approach--multimodal contrastive learning with joint example selection (JEST)--surpasses state-of-the-art models with up to 13$\times$ fewer iterations and 10$\times$ less computation. Essential to the performance of JEST is the ability to steer the data selection process towards the distribution of smaller, well-curated datasets via pretrained reference models, exposing the level of data curation as a new dimension for neural scaling laws.

==> Sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} We discuss the limitations in the Discussion Section.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{} We did not discuss potential negative societal impacts as our method does not relate to particular applications. The potential societal impacts are that better pre-training performance can be achieved with smaller computational resources, which we would consider positive.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{} We have read the guidelines and are confident that the paper adheres to the standards therein. We are not publishing a new dataset. We do not publish any images from or expose details of the datasets used that might compromise an individual. To the best of our knowledge, the datasets do not excarcerbate bias or contain any personally sensitive information.
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{} We do not include new theoretical results.
	\item Did you include complete proofs of all theoretical results?
    \answerNA{} We do not include new theoretical results.
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{} We do not explicitly provide the code for our experiments, however we detail in pseudo-code the main components of our method (see algorithms \ref{alg:sample_sigmoid} and \ref{alg:training_loop}). Our model implementations and base experimental configuration were adopted from the open source \texttt{big\_vision} codebase \cite{big_vision}. We do not provide the reference or downstream training datasets, but we provide ablations (see Experiments Section) on the open source LAION dataset.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} We describe and analyse experimentally the hyperparameters that relate specifically to our methods. We provide pseudocode for our method in the main text and Appendix, and describe all our hyperparameters. All other parameters are adopted from SigLIP pretraining in the \texttt{big\_vision} codebase \cite{big_vision,zhai2023sigmoid}. % If not described, experimental configuration was adopted from
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{} We do not publish error bars anywhere in the paper since we only publish single runs for all all experiments.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} Yes! This is a core contribution of the paper. All FLOP calculations are detailed in both the Methods and Experiments Section. Please refer to Table 2 for a summary of the computation associated with the main results, and Appendix \ref{sec:app-config} for a description of training resources. 
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} Yes, we cite the creators of the datasets and the code from which we forked our main model code.
  \item Did you mention the license of the assets?
    \answerNo{} We cannot share details of the reference model datasets.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{} We cannot release the datasets used for training in our study, but provide ablations with the open source LAION dataset. We consider the main contribution of our paper as conforming to the following category, taken from the Datasets and Benchmarks Call main page: ``Advanced practices in data collection and curation that are of general interest even if the data itself cannot be shared''.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{} We curate and train models on standard datasets (WebLI \cite{chen2022pali} and LAION \cite{schuhmann2022laion}), but we did not discuss details of how the datasets used were collected. %  are not releasing a new dataset
    % \answerYes{} We curate and train our models on Webli \cite{chen2022pali}, which was collected under strict
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{} Yes, Webli was specifically collected and filtered so as to % to our knowledge, the datasets used do 
    not contain any personally identifiable information or offensive content.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{} We do not use crowdsourced datasets with human subjects.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{} We do not use crowdsourced datasets with human subjects.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{} We do not use crowdsourced datasets with human subjects.
\end{enumerate}

\end{enumerate}

==> Tables/laion_table_orig.tex <==
\begin{table*}

\floatbox[{\capbeside\thisfloatsetup{capbesidesep=qquad}}]{table}
{
\caption{\textbf{Comparison to LAION pretraining.} JEST++ strongly surpasses prior art while requiring significantly fewer training iterations. COCO performance denotes the average of image-to-text and text-to-image retrieval. \vspace{0.5em}
}
\label{tab:test}}
{

\small 
 
\begin{tabular}{lcccc|c|cccc}

Method & \# Train & IN1K ZS & COCO \\

\hline

% Data goes here

LAION-440M \citep{radenovic2023filtering} & 12.8B & 64.1 & 48.1  \\ 
SemDeDup \citep{abbas2023semdedup} & 8.8B & 64.3 & 48.9 \\
DBP \citep{abbas2024effective} & 5.3B & 65.5 & 48.4 \\
DBP \citep{abbas2024effective} & 3.6B & 64.1 & 45.7 \\
SigLIP \cite{zhai2023sigmoid} & 1.3B & 57.2 & 43.3 \\
\rowcolor{DnCBG}JEST++ & \textbf{1.3B} & 
\textbf{66.8} & \textbf{54.8} \\

%

\end{tabular}
}
\vspace{-1em}
\end{table*}

==> Tables/main_table_bis.tex <==
\def\tbd{\textcolor{red}{TBD}}

% flops_per_image_siglip_B_16 = 35.1 * 3
% flops_per_image_jest_B_16 = 35.1 * (2 + 1 / SPI) if we cache the inference pass
%
% ratio = 7/3 = 2.333 for SPI = 0.2
%
% (3 * (0.5 * 1.0 + 0.5 * 0.25)) + 1 / SPI * 0.25
% = 3 * 0.625 + 0.25 * 5
% = 3.125
%
% = 1.042, so 4.2% overhead

\begin{table*}[h]
\centering
%\footnotesize
% \scriptsize
%\footscriptsize
\small

\newcommand*\rot{\rotatebox{90}}

% Paste output from Colab:
%   https://colab.corp.google.com/drive/1jYI-LEGIaf0gL5RTHff0IQwYVeu_m9MW?usp=sharing

\definecolor{goodgreen}{rgb}{0.25,0.7,0.25}
\definecolor{goodred}{rgb}{0.9,0.25,0.25}

\newcommand{\coloredcell}[3]{%
    \pgfmathsetmacro{\maxval}{#2}%
    \pgfmathsetmacro{\minval}{#3}%
    \pgfmathsetmacro{\scalar}{#1}%
    \pgfmathsetmacro{\range}{\maxval - \minval}%
    \pgfmathsetmacro{\normscalar}{(\scalar - \minval) / (\maxval - \minval) * 2 - 1}%
    \pgfmathsetmacro{\opacity}{100 * abs(\normscalar) * 0.8}%
    \ifdim\normscalar pt > 0pt
        \edef\tempcell{\noexpand\cellcolor{goodgreen!\opacity!white}}%
        \tempcell \scalar%
    \else
        \edef\tempcell{\noexpand\cellcolor{goodred!\opacity!white}}%
        \tempcell \scalar%
    \fi
}

\newcommand{\coloredcellpositive}[3]{%
    \pgfmathsetmacro{\textscalar}{#1}%
    \pgfmathsetmacro{\maxval}{#2}%
    \pgfmathsetmacro{\valscalar}{#3}%
    \pgfmathsetmacro{\normscalar}{\valscalar}%
    \pgfmathsetmacro{\opacity}{100 * log10(\valscalar) * 0.8}%
    \edef\tempcell{\noexpand\cellcolor{goodgreen!\opacity!white}}%
    \tempcell \textscalar%
}

\newcommand{\coloredcellnegative}[3]{%
    \pgfmathsetmacro{\textscalar}{#1}%
    \pgfmathsetmacro{\maxval}{#2}%
    \pgfmathsetmacro{\valscalar}{#3}%
    \pgfmathsetmacro{\normscalar}{\valscalar}%
    \pgfmathsetmacro{\opacity}{100 * log10(\valscalar) * 0.8}%
    \edef\tempcell{\noexpand\cellcolor{goodred!\opacity!white}}%
    \tempcell \textscalar%
}

% Paste here

\resizebox{\linewidth}{!}{

\begin{tabular}{lccc|c|cccccccc}
%\begin{tabular}{@{\extracolsep{1pt}}lccccccccccc|c@{}}


& & \multicolumn{2}{c}{FLOPs \%} &  & \multicolumn{2}{c}{ImageNet-1k} & \multicolumn{2}{c}{COCO} & & & & \\  % First row
%\cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
\cline{3-4} \cline{6-7} \cline{8-9}
&&&&&&&&&&&& \\ [-2ex]
%\noalign{\smallskip}
Method & \# Train & Per Iter. & \textbf{Total} & \textbf{Mean} & 10-S & ZS &  I2T & T2I & Birds & Caltech &  Cars & Pets \\% & $\mathbf{\Delta}$ \\  % Second row

% Method&\rot{FLOPs (\% Per Iter.)}&\rot{FLOPs (\% Total)}&\rot{Train Ex. (B)}&\rot{IN 10-Shot}&\rot{IN-1K}&\rot{COCO I2T R1}&\rot{COCO T2I R1}&\rot{Birds 10-Shot}&\rot{Caltech 10-Shot}&\rot{Cars 10-Shot}&\rot{Pets 10-Shot}&\rot{Mean}&$\Delta$ (\%)\\

\hline

CLIP \cite{radford2021learning}&13B&       100&\coloredcellpositive{32}{10.0}{3.08}&&&\coloredcell{68.3}{84.2}{69.2}&\coloredcell{52.4}{72.7}{57.7}&\coloredcell{33.1}{54.9}{39.9}&&&&\\
EVA-CLIP \cite{sun2023eva}&\hspace{0.5em}8B&       100&\coloredcellpositive{20}{10.0}{5.00}&&&\coloredcell{74.7}{84.2}{69.2}&\coloredcell{58.7}{72.7}{57.7}&\coloredcell{42.2}{54.9}{39.9}&&&&\\
OpenCLIP \cite{ilharco_gabriel_2021_5143773}&34B&       100&\coloredcellpositive{85}{10.0}{1.18}&&&\coloredcell{70.2}{84.2}{69.2}&\coloredcell{59.4}{72.7}{57.7}&\coloredcell{42.3}{54.9}{39.9}&&&&\\
LessIsMore \cite{cao2023less}&11B&       100&\coloredcellpositive{28}{10.0}{3.64}&&&\coloredcell{70.8}{84.2}{69.2}&\coloredcell{58.3}{72.7}{57.7}&\coloredcell{42.5}{54.9}{39.9}&&&&\\


SILC-S \cite{naeem2023silc}&20B&       380&
\coloredcellnegative{190}{10.0}{1.89}
%\edef\tempcell{\noexpand\cellcolor{goodred!0.53!white}}\tempcell 190%
&&\coloredcell{68.9}{77.8}{62.8}&\coloredcell{76.6}{84.2}{69.2}&\coloredcell{66.2}{72.7}{57.7}&\coloredcell{48.7}{54.9}{39.9}&&&&\\

SigLIP \cite{zhai2023sigmoid} &40B&       100&\coloredcellpositive{100}{10.0}{1.00}&\coloredcell{76.4}{78.9}{73.9}&\coloredcell{70.3}{77.8}{62.8}&\coloredcell{76.7}{84.2}{69.2}&\coloredcell{65.2}{72.7}{57.7}&\coloredcell{47.4}{54.9}{39.9}&\coloredcell{75.5}{83.0}{68.0}&\textbf{\coloredcell{92.8}{100.3}{85.3}}&\coloredcell{92.0}{99.5}{84.5}&\coloredcell{91.2}{98.7}{83.7}\\

% \vspace{-0.75em} \\ 


JEST&\hspace{0.5em}5B&       233&\coloredcellpositive{29}{10.0}{3.43}&\coloredcell{77.0}{78.9}{73.9}&\coloredcell{68.2}{77.8}{62.8}&\coloredcell{75.5}{84.2}{69.2}&\coloredcell{66.1}{72.7}{57.7}&\coloredcell{47.9}{54.9}{39.9}&\coloredcell{80.3}{83.0}{68.0}&\coloredcell{91.6}{100.3}{85.3}&\textbf{\coloredcell{93.3}{99.5}{84.5}}&\textbf{\coloredcell{93.3}{98.7}{83.7}}\\

Flexi-JEST&13B&       110&\coloredcellpositive{36}{10.0}{2.80}&\coloredcell{76.5}{78.9}{73.9}&\coloredcell{67.2}{77.8}{62.8}&\coloredcell{74.3}{84.2}{69.2}&\coloredcell{67.2}{72.7}{57.7}&\coloredcell{47.8}{54.9}{39.9}&\coloredcell{79.2}{83.0}{68.0}&\coloredcell{92.1}{100.3}{85.3}&\coloredcell{92.6}{99.5}{84.5}&\coloredcell{91.7}{98.7}{83.7}\\

JEST++&\hspace{0.5em}4B&       233&\coloredcellpositive{23}{10.0}{4.29}&\textbf{\coloredcell{78.2}{78.9}{73.9}}&\textbf{\coloredcell{70.3}{77.8}{62.8}}&\textbf{\coloredcell{76.9}{84.2}{69.2}}&\textbf{\coloredcell{70.3}{72.7}{57.7}}&\textbf{\coloredcell{53.3}{54.9}{39.9}}&\textbf{\coloredcell{80.4}{83.0}{68.0}}&\coloredcell{91.6}{100.3}{85.3}&\coloredcell{89.5}{99.5}{84.5}&\coloredcell{93.1}{98.7}{83.7}\\

Flexi-JEST++&\hspace{0.5em}4B&       110&\textbf{\coloredcellpositive{11}{10.0}{9.09}}&\coloredcell{76.7}{78.9}{73.9}&\coloredcell{68.2}{77.8}{62.8}&\coloredcell{75.8}{84.2}{69.2}&\coloredcell{68.0}{72.7}{57.7}&\coloredcell{51.2}{54.9}{39.9}&\coloredcell{78.8}{83.0}{68.0}&\coloredcell{91.6}{100.3}{85.3}&\coloredcell{88.5}{99.5}{84.5}&\coloredcell{91.8}{98.7}{83.7}\\



\end{tabular}
}
% End paste

%\end{tabular}
\vspace{1em}
\caption{\textbf{Comparison to prior art.} FLOP \% and colour gradients are measured relative to SigLIP \cite{zhai2023sigmoid}. Mean denotes the average performance over all metrics. ``Per Iter.'' denotes FLOPs per iteration. \talfan{Update}
}

\label{tab:main_table}
\end{table*}


==> Tables/rawvsfiltered_orig.tex <==
\begin{table}[h]

\definecolor{goodgreen}{rgb}{0.25,0.7,0.25}
\definecolor{goodred}{rgb}{0.9,0.25,0.25}

\pgfmathdeclarefunction{cliptoone}{1}{%
  \pgfmathparse{ifthenelse(#1 > 1, 1, ifthenelse(#1 < -1, -1, #1))}%
}

\newcommand{\coloredcell}[3]{%
    \pgfmathsetmacro{\maxval}{#2}%
    \pgfmathsetmacro{\minval}{#3}%
    \pgfmathsetmacro{\scalar}{#1}%
    \pgfmathsetmacro{\range}{\maxval - \minval}%
    \pgfmathsetmacro{\normscalar}{(\scalar - \minval) / (\maxval - \minval) * 2 - 1}%
    \pgfmathsetmacro{\clippednorm}{cliptoone(\normscalar * 0.8)}%
    \pgfmathsetmacro{\opacity}{100 * abs(\clippednorm) * 1.0}%
    \ifdim\normscalar pt > 0pt
        \edef\tempcell{\noexpand\cellcolor{goodgreen!\opacity!white}}%
        \tempcell \scalar%
    \else
        \edef\tempcell{\noexpand\cellcolor{goodred!\opacity!white}}%
        \tempcell \scalar%
    \fi
}
\newcommand{\coloredcellpositive}[3]{%
    \pgfmathsetmacro{\textscalar}{#1}%
    \pgfmathsetmacro{\maxval}{#2}%
    \pgfmathsetmacro{\valscalar}{#3}%
    \pgfmathsetmacro{\normscalar}{\valscalar}%
    \pgfmathsetmacro{\opacity}{100 * log10(\valscalar) * 0.8}%
    \edef\tempcell{\noexpand\cellcolor{goodgreen!\opacity!white}}%
    \tempcell \textscalar%
}

\newcommand{\coloredcellnegative}[3]{%
    \pgfmathsetmacro{\textscalar}{#1}%
    \pgfmathsetmacro{\maxval}{#2}%
    \pgfmathsetmacro{\valscalar}{#3}%
    \pgfmathsetmacro{\normscalar}{\valscalar}%
    \pgfmathsetmacro{\opacity}{100 * log10(\valscalar) * 0.8}%
    \edef\tempcell{\noexpand\cellcolor{goodred!\opacity!white}}%
    \tempcell \textscalar%
}

\floatbox[{\capbeside\thisfloatsetup{capbesidesep=qquad,capbesideposition= {right,center}}}]{table}
{
\caption{\textbf{Simplifying data curation.} All models are trained for 4B examples seen. Performance for JEST++ is nearly identical for pre-training on raw (uncurated) vs. filtered data. Color gradients are measured relative to IID training on filtered WebLI. \vspace{0.5em}
}
\label{tab:rawvsfilt}}
{
 
\small 
 
\begin{tabular}{lcccc|c|cccc}

Method & Filtered Data? & IN1K ZS & COCO \\

\hline

% Data goes here

\multirow{2}{*}{IID} & \checkmark & 73.6 & 52.5  \\ 
 & \xmark & \coloredcell{69.4}{83.6}{63.6} & \coloredcell{49.5}{62.5}{42.5} \\
\hline
\multirow{2}{*}{JEST++} & \checkmark & \coloredcell{76.9}{83.6}{63.6} & \coloredcell{61.8}{62.5}{42.5} \\
 & \xmark & \coloredcell{76.7}{83.6}{63.6}  & \coloredcell{61.8}{62.5}{42.5}  \\

%

\end{tabular}
}
\vspace{-1em}
\end{table}
